The 2025 Foundation Model Transparency Index

Foundation model developers are among the world's most important companies. As these companies become increasingly consequential, how do their transparency practices evolve? The 2025 Foundation Model Transparency Index is the third edition of an annual effort to characterize and quantify the transparency of foundation model developers. The 2025 FMTI introduces new indicators related to data acquisition, usage data, and monitoring and evaluates companies like Alibaba, DeepSeek, and xAI for the first time. The 2024 FMTI reported that transparency was improving, but the 2025 FMTI finds this progress has deteriorated: the average score out of 100 fell from 58 in 2024 to 40 in 2025. Companies are most opaque about their training data and training compute as well as the post-deployment usage and impact of their flagship models. In spite of this general trend, IBM stands out as a positive outlier, scoring 95, in contrast to the lowest scorers, xAI and Midjourney, at just 14. The five members of the Frontier Model Forum we score end up in the middle of the Index: we posit that these companies avoid reputational harms from low scores but lack incentives to be transparency leaders. As policymakers around the world increasingly mandate certain types of transparency, this work reveals the current state of transparency for foundation model developers, how it may change given newly enacted policy, and where more aggressive policy interventions are necessary to address critical information deficits.

==> appendices/app_selection.tex <==
\hypertarget{selection}{\section{Selection decisions}}
\label{app:selection}

In conducting the index, core structural design decisions are (i) the indicators used to assess developers and (ii) the developers that are assessed.
Here, we clarify both matters.
\subsection{Indicator selection}
\label{app:indicator-selection}
We use the same 100 indicators as FMTI v1.0 to facilitate direct comparison.
These indicators are listed by domain in \autoref{fig:indicators}.

\subsection{Developer selection}
\label{app:developer-selection}
We contacted 19 foundation model developers to request these developers submit transparency reports for the purpose of conducting FMTI v1.1.
Consistent with the principles used by \citet{bommasani2023fmti}, we only considered developers that are companies and that develop prominent foundation models.
Specifically, we contacted leadership via email at 01.ai, Adept, AI21 Labs, Aleph Alpha, Amazon, Anthropic, BigCode (Hugging Face and ServiceNow), Cohere, Databricks, Google, IBM, Inflection, Meta, Microsoft, Mistral, OpenAI, Stability AI, Writer, and xAI.
Following this email correspondence, and further clarification of the nature of the request, 14 foundation model developers agreed to provide the requested transparency reports.

Therefore, our selection process deliberately excluded foundation model developers that are not companies, even if they develop prominent foundation models, such as the Allen Institute for AI \citep[developer of models such as OLMo;][]{groeneveld2024olmo} and EleutherAI \citep[developer of Pythia;][]{biderman2023pythia}.
While developers such as AI2 and EleutherAI are often leaders in various types of transparency, releasing detailed information about data \citep{gao2020pile, soldaini2024dolma}, evaluations \citep{gao2021framework, magnusson2023paloma}, and the model development pipeline \citep{black2022neox, biderman2023pythia, groeneveld2024olmo}, we consider only companies in selecting developers to assess in FMTI v1.1. 

Our selection process also did not involve engagement with developers where we lacked connections with their leadership, which often coincides with models developed outside the United States and the Western hemisphere (\eg the developers of Falcon \citep{almazrouei2023falcon}, Qwen \citep{bai2023qwen}, DeepSeek \citep{deepseekai2024deepseek}, and HyperCLOVA \citep{yoo2024hyperclova}).

Finally, we did not engage any developer that released its first prominent foundation model during our execution of FMTI v1.1 (such releases include Apple's MM1 \citep{mckinzie2024mm1}, SambaNova's Samba 1 \citep{samba1}, Reka's Reka Core \citep{rekateam2024reka}, and Snowflake's Arctic-1 \citep{merrick2024arcticembed}). 
Moving forward, having successfully demonstrated that prominent foundation model developers have cooperated by submitting transparency reports, subsequent versions of the Foundation Model Transparency Index may engage these companies as well as others.
